Communication-efficient distributed eigenspace estimation with arbitrary node failures

We develop an eigenspace estimation algorithm for distributed environments with arbitrary node failures, where a subset of computing nodes can return structurally valid but otherwise arbitrarily chosen responses. Notably, this setting encompasses several important scenarios that arise in distributed computing and data-collection environments such as silent/soft errors, outliers or corrupted data at certain nodes, and adversarial responses. Our estimator builds upon and matches the performance of a recently proposed non-robust estimator up to an additive $\tilde{O}(\sigma \sqrt{\alpha})$ error, where $\sigma^2$ is the variance of the existing estimator and $\alpha$ is the fraction of corrupted nodes.

==> preamble.tex <==
\usepackage{latex-macros}
% \usepackage{mathpazo}
\usepackage{mathtools}
\usepackage{empheq}
\usepackage{multirow}
\usepackage[scale=0.75]{geometry}
\usepackage{booktabs}
\usepackage[capitalize]{cleveref}
\usepackage{amssymb,amsthm}
\usepackage[noend]{algpseudocode}
\usepackage{setspace}
\usepackage{appendix}
\usepackage{cancel}
\usepackage{diagbox}
\usepackage{enumitem}
\setlist[enumerate]{leftmargin=.3in}
\setlist[itemize]{leftmargin=.3in}
\usepackage{algorithm}
\usepackage{algpseudocode}
\usepackage[labelfont=bf]{caption}
\usepackage[sort,numbers]{natbib}
\usepackage{subcaption}
\usepackage{xfrac}
\usepackage{xcolor}
% Color palette using http://colorbrewer2.org/#type=diverging&scheme=RdBu&n=6
\definecolor{lblue}{HTML}{908cc0}
\definecolor{mblue}{HTML}{519cc8}
\definecolor{hblue}{HTML}{1d5996}
\definecolor{lred}{HTML}{cb5501}
\definecolor{mred}{HTML}{f1885b}
\definecolor{hred}{HTML}{b3001e}
\definecolor{ttred}{HTML}{ca3542}

\usepackage{tikz,pgfplots}
\pgfplotsset{compat=1.14}
\usetikzlibrary{automata,decorations.markings,positioning}

\newcommand{\bignorm}[1]{\bigl\| {#1} \bigr\|}
\newcommand{\bigopnorm}[1]{\bigl\| {#1} \bigr\|_{2}}
\newcommand{\biggnorm}[1]{\biggl\| {#1} \biggr\|}
\newcommand{\biggopnorm}[1]{\biggl\| {#1} \biggr\|_2}
\newcommand{\vasilis}[1]{{\color{blue} {#1}}}
\newcommand{\vcomment}[1]{{\color{blue} [\textbf{Vasilis}: {#1}]}}
\newcommand{\bsf}[1]{\textbf{\textsf{#1}}}

\crefname{appsec}{Appendix}{Appendices}

% build notes
% 1. delete old figure files (also maybe main.aux)
% 2. pdflatex
% 3. pdflatexmk


%\usepackage{sectsty}
%\allsectionsfont{\sffamily}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{proposition}{Proposition}

% need 'Assumption' theorem
\theoremstyle{definition}
\newtheorem{assumption}{Assumption}
\newtheorem{definition}{Definition}
\Crefname{assumption}{Assumption}{Assumptions}
\Crefname{theorem}{Theorem}{Theorems}
\Crefname{definition}{Definition}{Definitions}

\newcommand{\tsup}[1]{\textsuperscript{#1}}
\newcommand{\fbest}{f^{\mathrm{best}}}
\newcommand{\half}{\scalebox{0.65}}
\newcommand{\Lsym}{L_{\mathrm{sym}}}
\newcommand{\Esym}{E_{\mathrm{sym}}}
\newcommand{\Tmult}{T_{\mathrm{mult}}}
\newcommand{\mxhat}[2]{{\hat{{#1}}_{({#2})}}}
\newcommand{\est}{A}
\newcommand{\sol}{A}
\newcommand{\mtrv}{\widehat{V}}
\newcommand{\mtrz}{\widehat{Z}}
\newcommand{\mtry}{\widehat{Y}}
\newcommand{\mtrx}{\widehat{X}}
\newcommand{\err}{\widehat{E}}

\usepackage{hyperref}
\definecolor{mylinkcolor}{RGB}{0,0,140}
\hypersetup{colorlinks,allcolors=mylinkcolor,citecolor=mylinkcolor}

\title{Communication-efficient distributed eigenspace estimation with
arbitrary node failures}
\author{~%Vasileios Charisopoulos\thanks{
%Department of Operations Research \& Information Engineering,
%Cornell University, 14853 Ithaca NY - email: \url{vc333@cornell.edu}}
}

\delimiterfactor=750

\allowdisplaybreaks

